Fairness Transferability Subject to Bounded Distribution Shift

Given an algorithmic predictor that is "fair" on some source distribution, will it still be fair on an unknown target distribution that differs from the source within some bound? In this paper, we study the transferability of statistical group fairness for machine learning predictors (i.e., classifiers or regressors) subject to bounded distribution shifts. Such shifts may be introduced by initial training data uncertainties, user adaptation to a deployed predictor, dynamic environments, or the use of pre-trained models in new settings. Herein, we develop a bound that characterizes such transferability, flagging potentially inappropriate deployments of machine learning for socially consequential tasks. We first develop a framework for bounding violations of statistical fairness subject to distribution shift, formulating a generic upper bound for transferred fairness violations as our primary result. We then develop bounds for specific worked examples, focusing on two commonly used fairness definitions (i.e., demographic parity and equalized odds) and two classes of distribution shift (i.e., covariate shift and label shift). Finally, we compare our theoretical bounds to deterministic models of distribution shift and against real-world data, finding that we are able to estimate fairness violation bounds in practice, even when simplifying assumptions are only approximately satisfied.

==> Fairness Transfer Bounds-ArXiv3/Section/CovariateShift.tex <==
\section{Covariate Shift}
\label{sec:covariate-shift}
\vspace{-0.1in}
We now present our fairness transferability results subject to covariate
shift for both demongraphic parity (\Cref{sec:covariateDP}) and equalized opportunity (\Cref{sec:covariateEO}) as fairness criteria.
\subsection{Demographic Parity} \label{sec:covariateDP}

The simplest way to work with \cref{eq:v} is to bound the supremum \(v\). We first
consider demographic parity (\cref{eq:def-demographic-parity}) for
\(\mathcal{Y} = \{0,1\}\) and \(\mathcal{G} = \{g, h\}\), subject to covariate
shift (\cref{eq:def-covariate-shift}). We find that the form of \(\dispdp\)
subject to covariate shift recommends itself to a natural choice of vector divergence, \(\mathbf{D}\). \rr{First,} define a \emph{re-weighting coefficient} \(
 \omega_g(\R, \S, x) \define \frac{\Pr_{\R}(X {=} x \mid G {=} g)}{\Pr_{\S}(X {=} x \mid  G {=} g)}
\)\rr{.}
% From \cref{lem:cs-positive-prediction-rate-difference}, we obtain the following theorem
% \cref{lem:cs-positive-prediction-rate-difference} allows us to express the difference in positive prediction rate for \(\pi\) between \(\S\) and \(R\) by the covariate between the reweighting coefficient $\omega{w}_g(x)$ and the indicator of whether the policy makes a positive prediction on $x$ or not. We can then get the following bound on the fairness violation between the source and target distribution:
\begin{theorem}\label{thm:dp-covariate}
  For demographic parity between two groups under covariate shift (denoting, for
each \(g\), \(\beta_{g} \define \Pr_{\pi,\S}(\hat{Y} {=} 1 \mid G {=} g)\)), 
  \begin{equation}
    \disp_{\DP}(\pi, \R) \leq \disp_{\DP}(\pi, \S) + \sum_g
    \big(\beta_{g}(1 - \beta_{g}) \cdot \var_{\S}[\omega_g(\R, \S, x)]\big)^{\nicefrac{1}{2}}
  \end{equation}
\vspace{-0.1in}
\end{theorem}

We notice
that $\var_{\S}[\omega_g(\R, \S, x)]$ recommends itself as a suitable divergence
\(D_{g}\) from \(\S\) to \(\R\). Using basis vectors \(\mathbf{e}_g\), for this example, we could
define
\(
    \mathbf{D}(\mathcal{T} \parallel \S) = \sum_{g} \mathbf{e}_g
    \var_{\S}[\omega_g(\mathcal{T}, \S, x)]
\). % in which case we will require $\var_{\S}[\omega_g(\R, \S, x)] \leq B_g$.
    % Substituting this definition for \(\mathbf{D}\), we may write
% \begin{align} \label{eq:not-lipshitz}
% \begin{aligned}
%     \disp(\pi, \R) \leq& \\ \disp(\pi, \S) &+ \sum_g (\beta_{g})(1 - \beta_{g}) \mathbf{D}(\R \parallel \S)
% \end{aligned}
% \end{align}
% \yc{shall we use equation (48) as theorem 4.2's main result instead of (49)?} \rr{I commented out the equation I think you meant to deprecate. how does it read now?}
When \(\var_{\S}[\omega_g(\R, \S, x)] \leq B_g\), it follows
   $
    \disp_{\DP}(\pi, \R) \leq \disp_{\DP}(\pi, \S) + \sum_g
    \big(\beta_{g}(1 - \beta_{g}) \cdot B_g\big)^{\nicefrac{1}{2}}
$.
Comparing the inequality in
\cref{thm:dp-covariate}
% \cref{eq:not-lipshitz}
and the consequent of \cref{eq:lipshitz-upper}, we can interpret
\(\Pr_{\pi, \S}(\hat{Y} {=} 1)\) in \cref{thm:dp-covariate} as an upper bound for
the \emph{average} value of \(\nabla_{\mathbf{b}} v(\disp_\DP, \mathbf{D}, \pi, \R, \mathbf{b})\) along
any curve from \(\S\) to \(\R\). \rr{Interpreting} this result, the closer \({\rm Pr}(\hat{Y} {=} 1)\) is to 0.5 for
any group, the more potentially sensitive the fairness of the policy is to
distribution shifts for that group. We can further generalize the results to multi-class and multi-group setting:

\begin{corollary}\label{cor:dp-covariate-multi}
\cref{thm:dp-covariate} may be generalized to multiple classes
\(\mathcal{Y} = \{1, 2, ..., m\}\)
 and multiple groups \(\mathcal{G}\in\{1, 2, ..., n\}\), where \(\beta_{g,y} =\Pr(\hat{Y}{=}y \mid G{=}g)\) and assuming \(\var_{\S}[\omega_g(\R, \S, x)] \leq B_g\):
\begin{align}
  \dispdp(\pi, \R) &\define \sum_{y \in \mathcal{Y}} \sum_{g,h \in \mathcal{G}} \Big|
  \Pr_{\pi, \R}(\hat{Y} {=} y \mid G {=} g) -
  \Pr_{\pi, \R}(\hat{Y} {=} y \mid G {=} h)
  \Big| \\
  \disp_{\DP}(\pi, \R) &\leq \disp_{\DP}(\pi, \S) + \sum_{y} \sum_{g}
  \big(\beta_{g,y}(1 - \beta_{g,y}) \cdot B_g \big)^{\nicefrac{1}{2}}
\end{align}
\end{corollary}
We remark that in general, binary classification bounds may frequently be
generalized to multi-class bounds by redefining fairness violations as a sum
of binary-class fairness violations (\ie, same-class \vs different-class
labels) and summing the bounds on each.

\subsection{Equal Opportunity} \label{sec:covariateEO}

Consider an example using the \((Y {=} 1)\)-conditioned case
of Equalized Odds---termed \emph{Equal Opportunity} (\EOp). Denoting, for each group \(g\), the true positive rate
\(\beta^{+}_{g} \define \Pr_{\pi, \R}( \hat{Y} {=} 1 \mid Y {=} 1, G {=} g )\)
as an implicit function of \(\pi\) and \(\R\), we define disparity for \EOp as
\(
  \disp_\EOp(\pi, \R)
  \define \sum_{g, h \in \mathcal{G}}
 |
    \beta^{+}_{g} -
    \beta^{+}_{h}
 |
  % \disp_{\EOp}(\pi, \R) = \sum_{g, h \in \mathcal{G}}
  % \Big|
  % \TPR_g(\pi, \R) - \TPR_h(\pi, \R)
  % \Big|
\).
% where \(\beta^{+}_{g}\) is  for group \(g\).

We may bound the realized value of \(\disp_{\EOp}(\pi, \R)\) by bounding \(\beta^{+}_{g}\) for each group:
\begin{theorem} \label{thm:cov-EO-superbound}
 Subject to covariate shift and any given \(\mathbf{D}, \mathbf{B}\), assume extremal values for \(\beta_{g}^{+}\), \ie,
\begin{equation}
\label{eq:cov-EO-requisite}
\forall g, ~~
\big(D_{g}(\R \parallel \S) < B_{g}\big) \implies \big(
l_g \leq \beta^{+}_{g}(\pi, \R) \leq u_g\big)
\end{equation}
it follows that
\begin{equation} \label{eq:cov-eop-bound}
v(\disp_{\EOp}, \mathbf{D}, \pi, \S, \mathbf{B}) \leq \max_{\substack{{x_g \in \{l_g, u_g\}} \\ {x_h \in \{l_h, u_h\}}}} \sum_{g, h}\Big|
  x_g - x_h
\Big|
\end{equation}
\end{theorem}
\begin{corollary} \label{cor:max-cov-EO}
\rr{The disparity measurement} \(\disp_\EOp\) cannot exceed \(\frac{|\mathcal{G}|^2}{4}\).
\end{corollary}
In \cref{app:geometric}, we bound the extremal values of \(\beta_g^+\) by geometrically interpreting this quantity as an inner product on an appropriate vector space, utilizing the
freedom to select an appropriate \(\mathbf{D}\). 
%\vspace{-0.2in}


==> Fairness Transfer Bounds-ArXiv3/Section/Discussion.tex <==
\vspace{-0.1in}
\section{Conclusion and Discussion}
\vspace{-0.1in}
In this paper, we have developed a unifying framework for bounding the violation
of statistical group fairness guarantees when the underlying distribution
shifts within presupposed bounds. We hope that this work can
generate meaningful discussion regarding the viability of fairness guarantees
subject to distribution shift, the bounds of adversarial attacks against
algorithmic fairness, and evaluations of robustness with respect to algorithmic
fairness.
We believe that, just as published empirical measurements are of limited use without
reported uncertainties, fairness guarantees must be accompanied by bounds on their robustness to
distribution shift.

Future work remains to apply our framework for to problem of fairness transferability in settings with more complicated distribution shift dynamics. For example, compound distribution shifts \cite{schrouff2022maintaining}, which compose covariate shifts and label shifts, cannot be treated by composing the theoretical bounds developed herein without additional information regarding intermediate distributions. Another potential future direction is to develop reasonable bounds on
anticipated distribution shift from models of human behavior and exogenous
pressures.


==> Fairness Transfer Bounds-ArXiv3/Section/Formulation.tex <==
%\vspace{-0.1in}

\section{Formulation}\label{sec:formulation}
\emph{The \rr{appendices} include a table of notation (\cref{secA:notation}) and all proofs (\cref{app:proofs}).}
\vspace{-0.1in}
\subsection{Algorithmic Prediction}
\vspace{-0.05in}

We consider two distributions, \(\S\) (\emph{source}) and \(\R\)
(\emph{target}), each defined as a probability distribution for
\emph{examples}, where each example defines values for three random variables:
\(X\), a \textbf{feature} (\eg, \(x\)) with arbitrary domain \(\mathcal{X}\); \(Y\), a \textbf{label} (\eg, \(y\)) with arbitrary domain \(\mathcal{Y}\); and \(G\), a \textbf{group} (\eg, \(g\) or \(h\)) with finite, countable domain \(\mathcal{G}\). The predictor's policy \(\pi\), intended for \(\S\) but used on \(\R\), defines a fourth variable for each example: \viz, \(\hat{Y}\), a \textbf{predicted label} (\eg, \(\hat{y}\)) with domain \(\hat{\mathcal{Y}}
    = \mathcal{Y}\).
%% To motivate our discussion, consider the problem of whether to hire an applicant for a job performing skilled, independent tasks: \(X\) might represent an
%% applicant's credentials and scores from interviews; \(Y\), the ``true'' net
%% profit the company would make within the first year by hiring the applicant (or
%% alternatively, the ``correct'' hiring decision for the applicant); and
%% \(\mathcal{G}\), the zip code where the applicant was born. \yc{G represents the sensitive attribute?}

%% We train a predictor (classifier or regressor) to predict the value of \(Y\)
%% from \(X\) (and possibly \(G\)) in domain \(\D\) by using training
%% examples drawn independently from \(\D\). To represent the predictor's
%% estimate of \(Y\) on each example, we introduce a fourth random variable:

Using \(\mathcal{P}(\cdot)\) to denote the space of probability distributions
over some domain, we denote the space of distributions over examples
as \( \DD \define \mathcal{P}(\mathcal{X} \times \mathcal{Y} \times \mathcal{G}) \), such that \(\S, \R \in \DD\).
It will also be useful for us to notate the space of distributions over example
\emph{outcomes} associated with a given policy as
\( \OO \define \mathcal{P}(\mathcal{X} \times \mathcal{Y} \times \hat{\mathcal{Y}}) \)
and the space of distributions over of \emph{group-specific examples} as
\(\GG \define \mathcal{P}(\mathcal{X} \times \mathcal{Y})\).

%% In our example, the value of \(\hat{Y}\) corresponds to the predictor's estimate
%% of the profitability of hiring a given applicant (or alternatively, the
%% recommended hiring decision).

Without loss of generality, we allow the prediction policy \(\pi\) to be
stochastic, such that, for any combination \((x, g)\), the predictor effectively
samples \(\hat{Y}\) from a corresponding probability distribution \(\pi(x, g)\). %\yc{shall we add a sentence demonstrating the usefulness of stochastic classifier especially in the literature of fairness.} \rr{That is a great idea. Examples that come to mind are that \eg, threshold classifiers cannot always find non-trivial policies for DP or EO.}
Stochastic classifiers arise in various constrained optimization problems and \rr{proven useful} for making problems with custom losses or fairness constraints tractable \cite{cotter2019stochastic,grgichlaca2017fairness, narasimhan2018complex,wu2022metric}.

We denote the space of nondeterministic policies as
\(\Pi \define (\mathcal{X} \times \mathcal{G} \to \mathcal{P}(\hat{\mathcal{Y}}))\)
(\eg, \(\pi \in \Pi\)) and utilize the natural transformations that relate the spaces of distributions \(\DD\), policies \(\Pi\), and outcomes \(\OO\):
\begin{equation}\label{eq:pr-notation}
  \begin{aligned}
    \Pr_{\pi, \R}(\hat{Y} {=} \hat{y}, X {=} x, G {=} g) =
    \Pr_{\hat{Y} \sim \pi(x, g)}(\hat{Y} {=} \hat{y}) \cdot  \Pr_{X, G \sim \R}&(X {=} x, G {=} g)
  \end{aligned}
\end{equation}
%  \yc{should the first term of (6) be
% $\Pr_{\hat{Y} \sim \pi(x, g)}(\hat{Y} = \hat{y}| X = x, G = g)$?} \rr{No,
% because \(\pi\) returns a distribution for \(\hat{Y}\) only and loses
% information about \(X, G\)}\jl{We'd say $\pi$ is the distribution of $\hat{Y}$ only. And is Equation \ref{eq:pr-notation} used later?} \rr{Yes, and yes. Are you familiar with a better notation?}
% \yc{Notice that in Equation \ref{eq:pr-notation}, $\hat{Y}$ is sampled from $\pi(x, g)$, so once we have the policy $\pi(x,g)$, the distribution of $\hat{Y}$ will be independent of $x$ and $g$.}
We abuse the $\Pr$ notation for both probability
\emph{density} and probability \emph{mass} functions as appropriate.
% \rr{, and} for
% \emph{distributions} when the random variables inside the
% expression are~\rr{unspecified}.
%% To continue our example, it is possible that our predictor might yield different
%% outputs for identical candidates by design (e.g., as a way of managing risk,
%% representing uncertainty, or ``hedging our bets''); alternatively, the predictor
%% might be entirely deterministic, always producing identical outputs from
%% identical inputs. In either case, when we look at a sufficiently long list of
%% all (input, output) pairs of the predictor, we can reconstruct its effective
%% stochastic policy.
\vspace{-0.1in}
\subsection{Statistical Group-Fairness}
\vspace{-0.05in}

We next define a broad class of \emph{disparity} functions
\(
\disp \colon \Pi \times \DD \to \RR
\)
representing how ``unfair'' a given policy is for a given distribution
(\eg, writing \(\disp(\pi, \mathcal{T})\))\rr{, noting that this notion of fairness is} limited to capturing statistical discrepancies of outcomes between groups.
\begin{definition} \label{def:premetric} We define a \emph{premetric}\footnote{\rr{Despite use on Wikipedia, this is not a standard term in the literature. In general, the axioms of a premetric as defined in \cref{def:premetric} are a subset (thus ``pre'') of those that define a metric.}} \(\Psi\) on
  the space of distributions \(p\) with respect to \(q\)
  by the properties \(\Psi(p \parallel q) \geq 0\) and \(\Psi(p \parallel p) = 0\)
  for all \(p, q\), and refer to the value of \(\Psi\) as a ``shift''.
\end{definition}
\begin{definition} \label{def:disparity} 
  We define \rr{a} \emph{statistical group disparity} \(\disp\) for
  policy \(\pi\) and distribution \(\R\) in terms of the
  symmetrized shifts between group-specific outcome distributions. We measure shifts between outcome
  distributions with a given premetric
  \(
\Psi \colon \OO^2 \to \RR
  \).
  \begin{equation} \label{eq:premetric}
    \disp(\pi, \R) \define \sum_{g, h \in \mathcal{G}}
    \Psi \Big(
    \Pr_{\pi, \R}(X, Y, \hat{Y} \mid G {=} g) ~\big\|~
    \Pr_{\pi, \R}(X, Y, \hat{Y} \mid G {=} h)
    \Big)
  \end{equation}
%   \begin{align}
%     \label{eq:premetric}
%     \disp(\pi, \R) \define \sum_{g, h \in \mathcal{G}}
%     &\Psi \Big(
%     \PPh_g(\pi, \R)
%      ~\big\|~
%     \PPh_h(\pi, \R)
%       \Big) \\ \label{eq:def-Gamma}
%     \PPh_g(\pi, \R) &\define
%     \Pr_{\pi, \R}(X, Y, \hat{Y} \mid G = g)
% \end{align}
\end{definition}
%   Define    $, \Psi \colon \OO^2$ as one that satisfies Definition 2.1. Define $\PPh_g \colon \Pi \times \DD \to \OO$  such that $\PPh_g(\pi, \R) \define
%     \Pr_{\pi, \R}(X, Y, \hat{Y} \mid G = g)$ . Then  we define \emph{statistical group disparity} \(\disp\) in terms of the shifts
% between group-specific outcome distributions.
% %   \begin{equation} \label{eq:premetric}
% %     \disp(\pi, \R) \define \sum_{g, h \in \mathcal{G}}
% %     \Psi_{g,h} \Big(
% %     \hat{\mathbb{P}}_g(\pi, \R) ~\big\|~
% %     \hat{\mathbb{P}}_h(\pi, \R)
% %     \Big)
% %   \end{equation}
%   \begin{align}
%     \label{eq:premetric}
%     \disp(\pi, \R) \define \sum_{g, h \in \mathcal{G}}
%     &\Psi \Big(
%     \PPh_g(\pi, \R)
%      ~\big\|~  \PPh_h(\pi, \R)
%       \Big)\label{eq:def-Gamma}
% \end{align}
% where \(\hat{\mathbb{P}}_g(\pi, \R)\) represents the natural transformation of a
%   distribution of \(\R \in \DD\) and policy \(\pi \in \Pi\) to a
%   probability distribution over outcomes \((X, Y, \hat{Y})\) conditioned on
%   group \(G = g\).
% \begin{align}
%   \hat{\mathbb{P}}_g
%   & \colon \Pi \times \DD \to \mathcal{P}(\mathcal{X} \times \mathcal{Y} \times \hat{\mathcal{Y}}) \\
%   \hat{\mathbb{P}}_{g}[\pi, \R](x, y, \hat{y})
%   &= \Pr_{X, G, Y \sim \R}(X = x, Y = y, \pi(X, G) = \hat{y} \mid G = g)
% \end{align}
% and,
In \cref{def:disparity},
% \(\hat{\mathbb{P}}_g\) maps the policy \(\pi\) and distribution \(\R\) to the distribution of outcomes for group \(g\), while 
\(\Psi\) quantifies the \rr{specific} statistical differences in outcomes between groups that
are "unfair", where a value of 0 implies perfect fairness. In this work,
we assume that \(\Psi\) is the same for all \(g,h\) and that \(\disp\) is insensitive to relative group size \(\Pr(G)\).
\vspace{-0.1in}
\paragraph{Examples}
Familiar applications of \cref{def:disparity} include \emph{demographic parity}
(\DP) and \emph{equalized odds} (\EO). A policy satisfying \DP\rr{,
  in expectation, assigns
  a given binary classification \(y \in \{0, 1\}\) to the same fraction of examples in each group}. We may measure the
violation of \DP as
\begin{equation} \label{eq:def-demographic-parity}
\begin{multlined}
      \disp_\DP(\pi, \R)
      \define \sum_{g, h \in \mathcal{G}} \Big|
      \Pr_{\pi, \R}( \hat{Y} {=} 1 \mid G {=} g) - \Pr_{\pi, \R}( \hat{Y} {=} 1 \mid G {=} h)
      \Big|
\end{multlined}
\end{equation}
The associated \emph{premetric} \(\Psi_\DP\) \rr{for} \(p, q \in \OO\) is
$
  \Psi_\DP(p \parallel q) =
  \Big|
    \Pr_p(\hat{Y} {=} 1) - \Pr_q(\hat{Y} {=} 1)
  \Big|.
$
%\yc{$p$ and $q$ represent distributions?}\rr{Yes. Is there a way to make this more clear?}

To satisfy \EO, for binary \(\mathcal{Y} = \{0, 1\}\), \(\pi\) must maintain
group-invariant true positive and false positive classification rates.
We may measure the violation of \(\EO\) as
\begin{align}\label{eq:def-equalized-odds}
  \disp_\EO(\pi, \R)
  \define \sum_{g, h \in \mathcal{G}}
  \sum_{y \in \mathcal{Y}} \Big|
    \Pr_{\pi, \R}(\hat{Y} {=} 1 \mid G {=} g, Y {=} y) -
    \Pr_{\pi, \R}(\hat{Y} {=} 1 \mid G {=} h, Y {=} y)
  \Big|
\end{align}
The associated premetric is
$
  \Psi_\EO(p \parallel q) = \sum_{y \in \mathcal{Y}} \Big|
  \Pr_p(\hat{Y} {=} 1 \mid Y {=} y) - \Pr_q(\hat{Y} {=} 1 \mid Y {=} y)
  \Big|.
$
Note that the restriction of \EO to the \((Y = 1)\) case is known as \emph{Equal
Opportunity} (\EOp).

We remark that \cref{def:disparity} provides a unifying representation for a wide array of
statistical group ``unfairness'' definitions and may be used with inequality constraints.
That is, we may recover many working definitions of fairness that
effectively specify a maximum value of \rr{disparity}:
% \jl{What is the permissible fairness violation here? $d$ or $\epsilon$? If it is $\epsilon$, let's call it $\epsilon$-fair.}
% \rr{Yes, let's. Do you believe anything further should be done?} \jl{I believe $\epsilon$-fair is fine. I have revised $(d, \epsilon)$ appeared elsewhere.}
\begin{definition}
  A policy \(\pi\) is \textbf{\(\boldsymbol{\epsilon}\)-fair} with respect to \(\disp\)
  on distribution \(\R\) iff \(\disp(\pi, \R) \leq \epsilon\).
\end{definition}
\vspace{-0.1in}
\subsection{Vector-Bounded Distribution Shift}
% \begin{assumption}
% Suppose we develop an \(\epsilon\)-fair policy \(\pi\) for the source distribution
% \(\S\), \ie, \(\Delta^{\star}(\pi, \S) \leq \epsilon\).
% \end{assumption}
Suppose, after developing policy \(\pi\) for distribution \(\S\), we realize
some new distribution \(\R\) on which the policy is actually operating. This
realization may be the consequence of sampling errors during the learning
process, strategic feedback to our policy, random processes, or the reuse of our
policy on a new distribution for which retraining is impractical.
Our goal is to bound \(\disp(\pi, \R)\) given knowledge of \(\disp(\pi, \S)\)
and some notion of how much \(\R\) \rr{possibly} differs from \(S\).
% Let us define a
% vector-valued function \(\mathbf{D}\) on \(\DD^{2}\) with  group-specific
% components \(D_{g}\) that measure the shift in group-conditioned distributions
% of \(\Pr(X,Y\mid G{=}g)\) as \(\S\) mutates into \(\R\).
\begin{definition} \label{def:divergence}
  \(K(p \parallel q)\) is a \emph{divergence} if and only if for all \(p\) and \(q\), \(K(p \parallel q) \geq 0\) and \(K(p \parallel q) = 0 \iff q = p\).
\end{definition}
\begin{definition} \label{def:vector-divergence}
  Define the group-vectorized shift \(\mathbf{D}\), as \(\S\) mutates into \(\R\), as
  \begin{equation}
    \mathbf{D}(\R \parallel \S) \define \sum_g \mathbf{e}_g D_{g}\big(
    \Pr_{\R}(X, Y \mid G {=} g)
    \parallel
    \Pr_{\S}(X, Y \mid G {=} g)
    \big)
\end{equation}

where \(\mathbf{e}_{g}\) represents a unit vector indexed by \(g\), and each
\(D_{g} \colon \GG^{2} \to \RR\) is a divergence \rr{(\cref{def:divergence})}. Note that each \(D_g\) also defines a premetric (but not necessarily a divergence) on \(\DD\).
% and
% \(\mathbb{P}_g\) represents the natural transformation of a distribution that
% conditions the distribution on a given group \(G = g\).
% \begin{align}
%   \mathbb{P}_g
%   &\colon \DD \to
%   \mathcal{P}(\mathcal{X} \times \mathcal{Y}) \\
%   \mathbb{P}_g(\R)[x, y] &= \Pr_{X,Y,G \sim \R}\Big(X = x, Y = y \mid G = g\Big)
% \end{align}
\end{definition}
\begin{assumption} \label{asm:budget}
Let there exist some vector \(\mathbf{B} \succeq 0\) bounding \(\mathbf{D}(\R \parallel \S) \preceq \mathbf{B}\), where \(\preceq\)
and \(\succeq\) denote element-wise inequalities.
\end{assumption}
In \cref{asm:budget}, \(\mathbf{B}\) limits the possible distribution shift as
\(\S\) mutates into \(\R\), without requiring us to specify a model for how
distributions evolve. When modelling distribution shift requires complex dynamics (\eg, when agents learn and respond to classifier policy), we reduce a potentially difficult dynamical problem to a more tractable, adversarial problem to achieve a bound.
\begin{lemma} \label{lem:v-of-B0-is-R}
  For all \(\pi\), \(\disp\), and \(\mathbf{D}\), when \(\mathbf{B} = 0\),
\(\disp(\pi, \S) = \disp(\pi, \R)\).
\end{lemma}
\cref{lem:v-of-B0-is-R} indicates that, for a fixed policy \(\pi\), a change
in disparity requires a measurable shift in distributions \rr{from $\S$ to $\R$}, confirming intuition.
\vspace{-0.1in}
\paragraph{Restricted Distribution Shift}
Common assumptions that restrict the set of  distribution shifts include \emph{covariate shift} and \emph{label shift}.
For covariate shift, the distribution of \emph{labels} conditioned on \emph{features} is preserved across distributions for all groups, while for label shift, the distributions of \emph{features} conditioned on \emph{labels} is preserved across distributions for all groups.
\begin{align} \label{eq:def-covariate-shift}
\text{\textbf{Covariate shift} implies }&\Pr_{\R}(Y \mid X, G) = \Pr_{\S}(Y \mid X, G) \\
\label{eq:def-label-shift}
\text{\textbf{Label shift} implies }& \Pr_{\R}(X \mid Y, G) = \Pr_{\S}(X \mid Y, G)
\end{align}
%% For both Label Shift and Covariate Shift, we assume that decision subjects do
%% not change group membership (from $g$ to $h$ or vice-versa) despite the
%% distribution shift.
% \yl{Suggested organization
% \begin{itemize}
%     \item Section 3 would be only the general bounds
%     \item Section 4 Covraite shift with DP and EO (subsection: strategic classification as an example)
%     \item Section 5 Label shift with DP and EO (subsection: replicator dynamics as an example, rederive the bounds using the replicator dyanmics equation, use utility functions)
% \end{itemize}}
In \cref{sec:covariate-shift}, we explore a deterministic model of a population's response to classification \rr{as an example of} covariate shift. We do the same in \cref{sec:labelDP} for label shift.


==> Fairness Transfer Bounds-ArXiv3/Section/GeneralBound.tex <==
\vspace{-0.1in}
\section{General Bounds}\label{sec:bounds}
\vspace{-0.1in}
We first define a primary bound in \cref{def:v} before considering simplifying special cases.

Given an element-wise bound \(\mathbf{B}\) on the vector-valued shift
\(\mathbf{D}(\R \parallel \S)\) (\cref{asm:budget}) we may bound the disparity
\(\disp\) of policy \(\pi\) on any realizable target distribution \(\R\) by its supremum value.
\begin{definition} \label{def:v}
  Define the supremum value \(v\) for \(\disp\) subject to
\(\mathbf{D}(\R \parallel \S) \preceq \mathbf{B}\) as
\begin{align} \label{eq:v}
v(\disp, \mathbf{D}, \pi, \S, \mathbf{B})
  &\define
  \sup_{ \mathbf{D}(\R \parallel \S) \preceq \mathbf{B}} \disp(\pi, \R)\\
 \label{eq:mainresult}
  \mathbf{D}(\R \parallel \S) \preceq \mathbf{B}
  &\implies
  \disp(\pi, \R)
  \leq
  v(\disp, \mathbf{D}, \pi, \S, \mathbf{B})
\end{align}
\end{definition}
% Note that, for all possible target distributions \(\S \in \DD\),
% \begin{align}
%   v(\pi, \S, \mathbf{0}) &= \disp(\pi, \S) \\
%   \label{eq:posgrad}
%   \mathbf{B} \preceq \mathbf{C} &\implies v(\pi, \R, \mathbf{B}) \leq v(\pi, \R, \mathbf{C})
%   %TODO Prove when we have extra space
% \end{align}

% We note that lower bounds on \(\disp(\pi, \R)\) may be obtained by replacing the
% supremum in \cref{eq:v} with an infimum, possibly in combination with lower
% bounds on the shift \(\mathbf{D}(\R \parallel \S)\). In general, however,
% such lower bounds allow for \emph{reduced} fairness violation on the target
% distribution, \ie, \(\disp(\pi, \R) < \disp(\pi, \S)\), offering limited utility
% for the purpose of mitigating worst-case outcomes. Nonetheless, we provide an
% example lower bound in \cref{sec:lipshitz}.

In general, our strategy is to exploit the mathematical structure of the setting
encoded by \(\disp\) (\ie, \(\Psi\)) and \(\mathbf{D}\) to obtain an
upper bound for \(v\) defined in \cref{eq:v}. We first explore general cases of
simplifying assumptions before presenting worked special examples for frequently
encountered settings. Finally, we compare the resulting theoretical bounds to
numerical results and simulations.
\vspace{-0.1in}
\subsection{Lipshitz Conditions}
\label{sec:lipshitz}
The value of \(v\) defines a scalar field in \rr{\(\mathbf{B}\) and therefore} a conservative vector field \(\mathbf{F} = \nabla_{\mathbf{B}} v\). 
%\yl{didn't find $\mathbf{b}$ to be properly defined. or is it simply a variable? looks like each $b_i$ represents the shift for group $i$'s direction}

\begin{wrapfigure}{r}{.4\linewidth}
   \centering \includegraphics[width=\linewidth]{images/lipshitz_bound.pdf}
   \caption{A Lipshitz bound for all curves \rr{parameterized by distribution shift bound \(\mathbf{b}\)} in the \((0, \mathbf{B})\) \(\DD\)-hyperrectangle \rev{on the surface \(v\). In the figure, for groups \(i \in \{g, h\}\), \(\max \partial_i v = L_i\), and the colored dotted lines corresponds to \(L_i  b_i\), which, when summed, equal \(\mathbf{L} \cdot \mathbf{B}\). }}
 \label{fig:lipshitz}
\end{wrapfigure}
For any curve in \(\DD\) from \(\S\) to \(\R\), bounds of
the form \(\mathbf{F} \preceq \mathbf{L}\) for some constant \(\mathbf{L}\) along the curve imply a Lipshitz bound on \(\disp\). We visualize a bound in \cref{fig:lipshitz} for all possible curves in the region \(\mathbf{D}(\R \parallel \S) \preceq \mathbf{B}\).
\begin{theorem}[Lipshitz Upper Bound] \label{thm:lipshitz} If there exists an \(\mathbf{L}\) such that
\(
   \nabla_{\mathbf{b}} v(\disp, \mathbf{D}, \pi, \S, \mathbf{b}) \preceq \mathbf{L}
\),
everywhere along some curve \rr{as \(\mathbf{b}\) varies} from \(0\) to \(\mathbf{B}\), then
\begin{equation}
  \begin{aligned} \label{eq:lipshitz-upper}
  \disp(\pi, \R) \leq \disp(\pi, \S) + \mathbf{L} \cdot \mathbf{B}
\end{aligned}
\end{equation}
\end{theorem}
\rev{Succinctly, if we are guaranteed that disparity can never increase faster than a certain rate in some measure of distribution shift, then, given a maximum distribution shift, this rate bounds the maximum possible disparity.}
The utility of \cref{thm:lipshitz} arises when a Lipshitz condition \(\mathbf{L}\) is
known, but direct computation of \(v\)
is difficult. We provide an example of a Lipshitz bound in \cref{sec:labelDP}.


% \begin{corollary}[Lipshitz Lower Bound] \label{thm:lipshitz-lower} Extending \cref{thm:lipshitz}, if, in addition, \(\mathbf{D}\) is symmetric, \ie, for all \(p, q\),
% \(\mathbf{D}(p \parallel q) = \mathbf{D}(q \parallel p)\),
% then
% \begin{equation}
%   \disp(\pi, \R) \geq \disp(\pi, \S) - \mathbf{L} \cdot \mathbf{B}
% \end{equation}
% \end{corollary}


% \begin{theorem}[Lipshitz Lower Bound] \label{thm:lipshitz-lower} If
%   \begin{align}
%     \mathbf{D}(\R \parallel \S) &\preceq \mathbf{B} \implies
% \nabla_{\mathbf{b}} v(\pi, \R, \mathbf{b}) \preceq \mathbf{L} \\
% \forall p,q,~~ \mathbf{D}(p \parallel q) &= \mathbf{D}(q \parallel p)
%   \end{align}
% then
% \begin{equation}
%   \begin{aligned}
%     \mathbf{D}(\R \parallel \S) \preceq \mathbf{B} &\implies \\
%   \disp(\pi, \R) \geq \disp(\pi, \S) &- \mathbf{L} \cdot \mathbf{B}
% \end{aligned}
% \end{equation}
% \end{theorem}
% \yc{would it be possible to combine the above two theorems?} \rr{I made an
% attempt at compression; how does it read to you?}\jl{At least looks good to me.}
% \subsection{Subadditive Conditions} \label{sec:subadditive}
\subsection{Subadditivity Conditions}
\label{sec:subadditive}
\begin{definition} \label{def:w}
  Define $w$ as the maximum \emph{increase} in disparity
subject to \(\mathbf{D}(\R \parallel \S) \preceq \mathbf{B}\), \ie,
\(w(\disp, \mathbf{D}, \pi, \S, \mathbf{B}) \define v(\disp, \mathbf{D}, \pi, \S, \mathbf{B}) - \disp(\pi,\S)\).
\end{definition}

\begin{theorem} \label{thm:subadditive}
  Suppose, in the region \(\mathbf{D}(\R \parallel \S) \preceq \mathbf{B}\), that
  \(w\) is subadditive in its last argument.
That is,
\(
    w(..., \mathbf{a}) + w(..., \mathbf{c})
    \geq w(..., \mathbf{a} + \mathbf{c})
    \) for \(\mathbf{a}, \mathbf{c} \succeq 0\) and \(\mathbf{a} + \mathbf{c} \preceq \mathbf{B}\).
If \(w\) is also locally differentiable, then a first-order approximation of \(w(..., \mathbf{b})\) evaluated at
\(0\), \ie,
\begin{equation}
  \mathbf{L} =
  \nabla_{\mathbf{b}} w(..., \mathbf{b}) \big|_{\mathbf{b} = 0} =
  \nabla_{\mathbf{b}} v(..., \mathbf{b}) \big|_{\mathbf{b} = 0}
 \end{equation}
 provides an upper bound for \(v(..., \mathbf{B})\), \ie,
 \begin{equation}
   v(\disp, \mathbf{D}, \pi, \S, \mathbf{B})
   \leq
   \disp(\pi, \S) + \mathbf{L} \cdot \mathbf{B}
\end{equation}
\end{theorem}
\cref{thm:subadditive} notes that ``diminishing returns'' in the change of \(\disp\) as the
difference of \(\R\) with respect to \(\S\) is increased implies a bound on \(\disp\) in terms of its local sensitivity to \(\mathbf{D}\) at \(\S\) (\ie, using a first-order Taylor approximation). Note that, if \(w\) is concave in the bounded region, it is also subadditive in the bounded region, but the converse is not true, nor does the converse imply Lipshitzness.
% \subsubsection{Group-Subadditivity}\label{sec:groupsubadditivity}

% The last step in the above calculation (from \cref{eq:subadditive2} to
% \cref{eq:subadditive1}) corresponds to the subadditivity of \(w\) over
% group-specific domain shifts. While we will not explore an example of full
% subadditivity, we will use examples that satisfy the weaker condition of
% group-subaddivity, for which we may bound \(w\) subject to some group-specific
% shift, and compose such bounds additively:

% \begin{align}
%   w(\pi, \S, \mathbf{B}) \leq \sum_{g} w(\pi, \S, B_{g} \mathbf{e}_{g})
% \end{align}
% In particular, demographic parity (\cref{sec:labelDP}) and equal
% opportunity (\cref{sec:covariateEO}) are amenable to such bounds.
\vspace{-0.1in}
\subsection{Geometric Structure} \label{sec:metricbounds}

It may happen that \(\Psi \colon \OO^2 \to \RR \) and each
\(D_{g} \colon \GG^2 \to \RR \) share structure that permits a geometric
interpretation of distribution shift. While the utility of this observation
depends on the specific properties of \(\Psi\) and \(\mathbf{D}\), we
demonstrate a worked example building on \cref{sec:covariateEO} in
\cref{app:geometric}, in which we allow ourselves to select a suitable
\(\mathbf{D}\) for ease of interpretation. We proceed to consider worked examples that adopt common  assumptions
limiting the form of distribution shift and apply common definitions of statistical
group fairness.
%vspace{-0.1in}
%% \paragraph{Alternate Derivation}
%% From the definition of label shift we have for each group $g$:
%% %\yc{this should hold for each group $g$}
%% \begin{align*}
%%     \Pr_{\R}(X=x,Y=y|G = g) &=  \Pr_{\R}(X=x|Y=y, G = g) \cdot  \Pr_{\R}(Y=y, G = g)= \Pr_{\S}(X=x|Y=y, G = g) \cdot  \Pr_{\R}(Y=y,G = g)
%% \end{align*}
%% In the case of binary classification, let $p^g = \Pr_{\S}(Y=+1 | G=g)$ denote the positive label probability of group $g \in G$ under the target distribution. Similarly, let $\omega^g(h)$ denote the aggregate adaptation within group $a$ induced by a classifier $h$ trained on $\S$:
%% \begin{align*}
%%     \omega^g(h) := \Pr_{\R}(Y=+1 | G=g)
%%     \quad \mathrm{and} \quad
%%     1-\omega^g(h) = \Pr_{\R}(Y=-1 | G=g)
%% \end{align*}


%--------------------------------
%% \paragraph{Useful Lemmas}
%% For a particular group $g \in G$, define the true positive rate and false positive rate before and after induced distribution shift:
%% \begin{align*}
%%     \TPR^g_S(h): = \Pr_{\S}(h(x)=+1 | Y=+1, G=g),
%%     \quad
%%     \TPR^g_h(h): = \Pr_{\R}(h(x)=+1 | Y=+1, G=g) \\
%%     \FPR^g_S(h): = \Pr_{\S}(h(x)=+1 | Y=-1, G=g),
%%     \quad
%%     \FPR^g_h(h): = \Pr_{\R}(h(x)=+1 | Y=-1, G=g)
%% \end{align*}
%% We will make use of the following facts:

%% \begin{lem} \label{lem:label-shift-TPR-FPR}
%% Under label shift,  $\TPR^g_S(h) = \TPR^g_h(h)$ and $\FPR^g_S(h) = \FPR^g_h(h)$.
%% \end{lem}
%% \begin{proof}
%% We have
%% \begin{align*}
%%     \TPR^g_h(h) =& \Pr_{\R}(h(X) = +1|Y = +1, G=g)\\
%%     =& \int \Pr_{\R}(h(X) = +1, X= x|Y = +1, G=g)dx\\
%%     =& \int \Pr_{\R}(h(X) = +1| X= x,Y = +1, G=g) \Pr_{\R}(X= x | Y = +1, G=g)dx\\
%%     =& \int \Indicator[h(x) = +1] \Pr_{\R}(X= x | Y = +1, G=g)dx\\
%%     =& \int \Indicator[h(x) = +1] \Pr_{\S}(X= x | Y = +1, G=g)dx \tag{by definition of label shift}\\
%%     =& \int \Pr_{\S}(h(X) = +1| X= x,Y = +1, G=g) \Pr_{\S}(X= x | Y = +1, G=g)dx\\
%%     =& \TPR^g_S(h)
%% \end{align*}
%% The argument for $\FPR^g_h(h) = \FPR^g_S(h)$ is analogous.
%% \end{proof}

%% First, we can show that for each group $a\in A$, we can break the true prediction rate into a weighted combination of $\TPR^g$ and $\FPR^g$:
%% \begin{lem}
%% \label{lem: break of positive prediction}
%% $ \Pr_{\D} (h(x) = +1 | G=g) = \omega^g(h) \TPR^g(h) + (1 - \omega^g(h)) \FPR ^g(h)$ for a particular group $a \in A$ from an arbitrary distribution $\D$, where the weighted term $\omega^g(h) = \Pr_{\D}(Y = +1|  G=g)$.
%% \begin{proof}
%% \begin{align*}
%%     \Pr_{\D} (h(x) = +1 | G=g) &= \sum_{y\in \{0,1\}}\Pr_{\D}(h(x) = +1, Y = y | G=g) \\
%%     &= \sum_{y\in \{0,1\}}\Pr_{\D}(h(x) = +1| Y = y,  G=g)\Pr_{\D}(Y = y|  G=g) \\
%%     &=\omega^{a}(h)\TPR^g_{\D}(h) +(1-\omega^{a}(h))\FPR^g_{\D}(h)
%% \end{align*}
%% \end{proof}
%% \end{lem}

%% We can also bound the difference between the true prediction rate before and after deployment of a model $h$. Recall $p^g = \Pr_{\S}(h(x) = +1 | G=g)$:

%% \begin{lem}
%% \label{lem: change in positive prediction}
%% $\Pr_{\S}(h(x) = +1|G=g) - \Pr_{\R}(h(x) = +1|G=g) =  (p^g(h) - \omega^g(h)) (\TPR^g(h) - \FPR^g(h)) $
%% \end{lem}
%% \begin{proof}
%% \begin{align*}
%%    &\Pr_{\S}(h(x) = +1|G=g) - \Pr_{\R}(h(x) = +1|G=g)\\
%%    =& (p^g(h) \TPR_S^g(h) + (1-p^g(h)) \FPR_S^g(h)) - (\omega^g(h) \TPR_h^g(h) + (1-\omega^g(h)) \FPR_h^g(h))  \tag{By lemma \ref{lem: break of positive prediction}}\\
%%    =&  (p^g(h) - \omega^g(h)) (\TPR^g(h) - \FPR^g(h))
%% \end{align*}
%% \end{proof}

%% Thus we can compute the demographic parity between two groups after distribution shift as:
%% \begin{align}
%%     \Delta_\DP^{\R}(h) &= |\Pr_{\R}(h(x) = +1 | G=g) -\Pr_{\R}(h(x) = +1 | G = b) | \nonumber \\
%%     &= \Big|\Pr_{\R}(h(x) = +1 | G=g) - \Pr_{\S}(h(x) = +1 | G=g) \nonumber \\
%%     & \qquad \qquad  + \underbrace{\Pr_{\S}(h(x) = +1 | G=g)- \Pr_{\S}(h(x) = +1 | A = b)}_{\epsilon^{\S}_\DP} \nonumber \\
%%     & \qquad \qquad  + \Pr_{\S}(h(x) = +1 | A = b) - \Pr_{\R}(h(x) = +1 | G = b) \Big| \tag{Add and substract terms} \nonumber \\
%%     &= \Big|(\omega^a(h) - p^a(h))(\TPR^a(h) - \FPR^a(h)) - (\omega^b(h) - p^b(h))(\TPR^b(h) - \FPR^b(h)) + \epsilon^{\S}_\DP(h)\Big|
%%     \tag{By Lemma \ref{lem: change in positive prediction}}
%% \end{align}


%% \paragraph{Bounds}
%% \begin{itemize}
%%     \item Upper bound: From the above derivation of $\Delta_\DP^{\R}(h)$ we can get an upper bound as:
%%     \begin{align*}
%%         \Delta_\DP^{\R}(h)\leq \Delta^{\S}_\DP(h) + \Big|(\omega^g(h) - p^g(h))(\TPR^g(h) - \FPR^g(h)) \Big| + \Big|(\omega^g(h) - p^g(h))(\TPR^b(h) - \FPR^b(h))\Big|
%%     \end{align*}
%%     \item Lower bound?
%%     \rr{claim:
%%     \[
%%     \Delta_\DP^{\R}(h)\geq \Delta^{\S}_\DP(h) -  \sum_g \Big|(\omega^g(h) - p^g(h))(\TPR^g(h) - \FPR^g(h)) \Big|
%%     \]
%%     since \(\Delta_{DP}\) can't decrease by more than the sum of absolute values
%%     }
%% \end{itemize}

%% #//  ____        _               _     _ _ _   _
%% #// / ___| _   _| |__   __ _  __| | __| (_) |_(_)_   _____
%% #// \___ \| | | | '_ \ / _` |/ _` |/ _` | | __| \ \ / / _ \
%% #//  ___) | |_| | |_) | (_| | (_| | (_| | | |_| |\ V /  __/
%% #// |____/ \__,_|_.__/ \__,_|\__,_|\__,_|_|\__|_| \_/ \___|
%% #//


==> Fairness Transfer Bounds-ArXiv3/Section/Introduction.tex <==
\section{Introduction}

\emph{Distribution shift} is a common, real-world phenomenon that affects
machine learning deployments when the \emph{target} distribution of examples
(features and labels) \rr{ultimately} encountered by a \rr{data-driven} policy diverges from the
\emph{source} distribution it was trained for. For socially consequential
decisions guided by machine learning, such shifts in the underlying distribution
can invalidate fairness guarantees and cause harm by exacerbating social
disparities.
Unfortunately, distribution shift can be technically difficult or impossible to
model at training time \rr{(\eg, when depending on complex social dynamics or
unrealized world events)}.
Nonetheless, we still wish to
certify the robustness of fairness \rr{metrics for} a policy on possible target
distributions.

In this paper, we provide a general framework for quantifying the robustness of statistical group fairness
guarantees.
We assume that the target distribution is \rr{adversarially} drawn from a bounded
domain, thus reducing the hard problem of modelling distribution shift dynamics
to a more tractable, \rr{static} problem. \rr{With this framework, we
  can detect potentially inappropriate policy applications, prior to deployment, when
  fairness violation bounds are not sufficiently small}.


This work bridges a gap between recent literature on \emph{domain adaptation},
which has largely focused on the transferability of prediction accuracy (rather
than fairness), and \emph{algorithmic fairness}, which has typically
considered static distributions or prescribed models of
distribution shift. Our work is the first to systematically bound quantifiable
violations of statistical group fairness while remaining agnostic to (1) the
mechanisms responsible for distribution shift, (2) \rr{how group-specific
distribution shifts are quantified}, and (3) the specific statistical
definition of \rr{group} fairness applied.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
\begin{example}[htb]
    \centering
    \includegraphics[width=0.8\linewidth]{images/example-race-4.pdf}
    \caption{In \cref{sec:realcomparison}, we evaluate our bounds against
historical, temporal distribution shifts in demographics and income recorded by the US Census
Bureau~\cite{ding2021retiring}. The above figure depicts changes to accuracy and
fairness violation when a classifier initially trained on US state-specific data
for 2014 is reused on 2018 data, thus exemplifying the negative potential effects
of distribution shift.}
    \label{example:forecast-income}
      % and its effects on a classifier  is to predict an individual's income for 2018 while only accessing to training examples for 2014. We show the transferred accuracy and fairness violation of fair classifiers under demographic parity constraint. Each arrow represents the performance shift evaluated on data distribution corresponding to five US states, including California (CA), Michigan (MI), North Carolina (NC), Texas (TX), and Washington (WA). The arrow base represents the (accuracy, demographic disparity) point evaluated in year 2014, while the head represents the (accuracy, demographic disparity) point evaluated in year 2018.
\end{example}
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{wrapfigure}{r}{.44\linewidth}
    \centering
    %\captionsetup{width=\linewidth}
    \includegraphics[width=\linewidth]{images/example-2.pdf}
    \caption{In \cref{sec:realcomparison}, we evaluate our bounds against historical, temporal distribution shifts in demographics and income recorded by the US Census Bureau~\cite{ding2021retiring}. The above figure depicts changes to \rr{income-prediction} accuracy and \rr{demographic parity violation} when a classifier initially trained on US state-specific \rr{demographic} data for 2014 is reused on 2018 data, thus exemplifying the negative potential effects of distribution shift.}
    \label{example:forecast-income}
    % and its effects on a classifier  is to predict an individual's income for 2018 while only accessing to training examples for 2014. We show the transferred accuracy and fairness violation of fair classifiers under demographic parity constraint. Each arrow represents the performance shift evaluated on data distribution corresponding to five US states, including California (CA), Michigan (MI), Pennsylvania (PA), Texas (TX), and Washington (WA). The arrow base represents the (accuracy, demographic disparity) point evaluated in year 2014, while the head represents the (accuracy, demographic disparity) point evaluated in year 2018.
\end{wrapfigure}
Our primary result is a bound on a policy's potential ``violation of statistical
group fairness''\rr{---}defined in terms of the differences in policy outcomes between
groups\rr{---}when applied to a target distribution shifted relative to the source
distribution within known constraints.
\rr{Such settings naturally arise whenever training data represents a random
sample of a target population with different statistics or a sample from dynamic
environments, when a policy is reused on a new distribution without retraining, or
whenever policy deployment itself induces a distribution shift}.
\rr{As an example of this last case, strategic individuals
seeking loans might change their features or abstain from future application (thus shifting the distribution of
examples) in response to policies trained on historical data} \cite{hardt2016strategic, ustun2019actionable, zhang2020fair}. %We
%outline such a scenario with \cref{example:strategic-manipulation}. 
\rr{Beyond policy selection, exogenous pressure such as economic trends and noise
may also drive distribution shift in this example.}

In \cref{example:forecast-income}, we show how a real-world
distribution shift in demographic and income data for US states between 2014 and
2018 may increase fairness violations while decreasing accuracy for a
hypothetical classifier trained on the 2014 distribution. In such settings, it
is useful to quantify how fairness guarantees transfer across distributions
shifted within some bound, thus allowing the deployment of unfair machine
learning policies to be avoided.

\vspace{-0.1in}

% We next explore how bounds on distribution shift imply bounds on induced
% disparity, both in general and subject to simplifying assumptions.


% Where possible, we interpret our results, for example revealing clear trade-offs between accuracy and transferable fairness guarantees.

% several kinds of domain adaptation have been
% studied in the literature, including cases in which a predictor is simply reused
% on a new domain, or situations in which the distribution of examples actively
% changes in response to a predictor's policy. For example, in the ``strategic
% classification'' literature, individuals subject to algorithmic classification
% may strategically manipulate their features (e.g., falsifying income on a loan
% application) to receive more favorable classification (e.g., securing the loan),
% thereby shifting the relationship between features and labels (income and loan
% qualification) observed by the classifier \cite{hardt2016strategic}. In work on
% ``algorithmic recourse'', individuals may rationally invest in securing
% different labels (e.g., earning a degree) if given the belief that an existing
% classifier will recognize this change, leading to more positive outcomes
% \cite{ustun2019actionable}(see \Cref{fig:motivating-example-sc} for demonstration). In other work, individuals may elect whether to
% subject themselves to machine prediction (e.g., in recommendations systems), and
% the exodus of dissatisfied users can change the distribution of users observed
% by the predictor \cite{zhang2020fair}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% MOTIVATING EXAMPLES
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \iffalse
% \begin{figure}[!thb]
% \begin{minipage}[t]{\textwidth}
%     % define the example environment
%     \floatstyle{ruled}
%     \newfloat{example}{thp}{lop}
%     \floatname{example}{Example}
%     \centering
%     \begin{minipage}[t]{0.45\textwidth}
%         \includegraphics[width=\textwidth]{images/example-race-4.pdf}
%         \captionsetup{type=example}
%         \vspace{-0.2in}
%         \captionof{example}{We investigate temporal domain shift on ACS Income data~\cite{ding2021retiring}. We show the transferred accuracy and fairness violation of fair classifiers under demographic parity constraint. Each arrow represents the data distribution corresponding to different US states, including California (CA), Michigan (MI), North Carolina (NC), Texas (TX), and Washington (WA). The arrow base represents the (accuracy, demographic disparity) point evaluated in year 2014, while the head represents the (accuracy, demographic disparity) point evaluated in year 2018.}
%     \end{minipage}
%     \hfill
%     \begin{minipage}[t]{0.50\textwidth}
%         \centering
%         \includegraphics[width=0.8\textwidth]{images/strategic_classification_motivating_example.pdf}
%         \captionsetup{type=example}
%         \captionof{example}{We demonstrate an example of distribution shift as a result of decision subjects' agency: when the decision subjects observe the decision rule (the green line in the figure), they will adapt their feature in order to get a more favorable prediction outcome. In this example, when the decision subject observe that both credit score and income are deciding factors of the decision rule, they will try to improve both features efficiently (i.e. they will along the direction that is perpendicular to the decision rule).This is known as \emph{strategic manipulation} \cite{hardt2016strategic}.}
%         % \label{fig:motivating-example-sc}
%     \end{minipage}
%     \label{fig:motivating-examples}
% \end{minipage}
% \end{figure}
% \fi
% \yl{move Example 2 to appendix}
% \yl{leave the full related work to appendxi too. shorten \& summarize it here}
\vspace{-0.05in}
\subsection{Related Work}
\vspace{-0.1in}
% \rr{notes from meeting:}
% \begin{enumerate}
%  \item Achievability of fairness guarantees
%  \item Quantifying effects of distribution shift
%  \begin{itemize}
%     \item FACCT 2021 paper - DP covariate shift
%  \end{itemize}
%  \item Modelling domain adaptation of populations
% \end{enumerate}

% related work in domain adaptation
Our work \rr{considers} a setting similar \rr{to} recent \rr{studies of}
\emph{domain adaptation}, which have largely focused on characterizing the
effects of distribution shift on prediction performance rather than fairness.
\rr{Our work also} builds on \rr{efforts in} \emph{algorithmic fairness},
\rr{especially \emph{dynamical} treatments of distribution shift in response to deployed machine learning policies} \cite{liu2018delayed,creager2020causal, raab2021unintended}. 
%\yl{cite Reilly's paper}
We reference specific prior work in these domains in \cref{secA:related-work}\rr{, and here discuss existing work}
 that focuses on how certain measures of fairness are affected when policies are subject to
specific distribution shift.

% add literature of fairness + domain adaptation
\textbf{Fairness subject to Distribution Shift:}
A number of recent studies have considered specific examples of
fairness transferability subject to distribution shift
\cite{schumann2019transfer, Coston2019fair, Singh2021fairness,rezaei2021robust, kang2022certifying}. 
% One focus of this topic is to provide theoretical bounds for the transferability
% of fairness violation \cite{schumann2019transfer}.  Such result is important
% because there are situations where model retraining data is too expensive or
% when we cannot have accessible data from the target domain.
In particular, \citet{schumann2019transfer} examine \emph{equality of
opportunity} and \emph{equalized odds} as definitions of group fairness subject
to distribution shifts quantified by an $\H$-divergence function; \citet{Coston2019fair}
consider \emph{demographic parity} subject to a \emph{covariate shift} assumption
while group identification remains unavailable to the classifier;
% https://dl.acm.org/doi/pdf/10.1145/3306618.3314236
\citet{Singh2021fairness} focus on common group fairness definitions for binary
classifiers subject to a class of distribution shift that generalizes covariate
shift and label shift by preserving some conditional probability between
variables; and
% https://dl.acm.org/doi/pdf/10.1145/3442188.3445865
\citet{rezaei2021robust} similarly consider common binary classification
fairness definitions \rr{such as equalized odds} subject to covariate
shift.
% https://www.aaai.org/AAAI21Papers/AAAI-8972.RezaeiA.pdf
While we address similar settings to these works as special cases of our bound,
we propose a unifying formulation for a broader class of statistical group fairness
definitions and distribution shifts. In doing so, we recognize that particular
settings recommend themselves to more natural measures of distribution shift,
providing examples in \cref{sec:covariateDP}, \cref{sec:covariateEO}, and
\cref{sec:labelDP}). 

\rr{Another thread in existing literature is the development of robust models with the goal of guaranteeing fairness on a modelled target distribution} (e.g., \cite{an2022transferring,Roh2021sample,mandal2020ensuring, biswas2021ensuring, kang2022certifying})
%\yl{cite the uiuc paper: Certifying Some Distributional Fairness with Subpopulation Decomposition
%}
, for example, by assuming covariate shift
and the availability of some unlabelled target data \cite{Coston2019fair,
  Singh2021fairness, rezaei2021robust}.
In particular, \citet{Singh2021fairness}
focus on learning stable models that will preserve prediction accuracy and
fairness, utilizing a causal graph to describe anticipated distribution
shifts. \citet{rezaei2021robust} takes a robust optimization
approach, and \citet{Coston2019fair} develops prevalence-constrained and
target-fair covariate shift method for getting the robust model. In contrast, our goal is to quantify fairness violations after an \emph{adversarial} distribution shift for \rr{\emph{any} given policy, including those not trained with robustness in mind}.

\vspace{-0.1in}
\subsection{Our Contributions}
\vspace{-0.1in}

Our primary contribution is formulating a general, \rev{worst-case} upper bound for a \rev{given} policy's
violation of statistical group fairness subject to group-dependent distribution
shifts \rev{within presupposed bounds} (i.e., \cref{eq:mainresult}).
Bounding
violations of fairness subject to distribution shift allows us to recognize and avoid potentially
inappropriate deployments of machine learning \rev{when the potential disparities of a prospective policy eclipse a given threshold within bounded distribution shifts of the training distribution.}

We first characterize the space of statistical
group fairness definitions and possible distribution shifts by appeal to
premetric functions (\cref{def:premetric}). \rr{After formulating the worst-case upper bound, we explore} common sets of
simplifying assumptions for this bound as special cases, yielding tractable
calculations for several familiar combinations of fairness definitions and
subcases of distribution shift (\cref{thm:dp-covariate}, \cref{thm:dp-label}) with
readily interpretable results. \rr{Finally,} we compare our theoretical bounds to
prescribed models of distribution shift in \cref{sec:syntheticcomparison} and to
real-world data in \cref{sec:realcomparison}. \rr{The details for reproducing our experimental results can be found at \\ {\small \texttt{\url{https://github.com/UCSC-REAL/Fairness_Transferability}}}.} 
%\vspace{-1em}



==> Fairness Transfer Bounds-ArXiv3/Section/Simulation.tex <==
\vspace{-0.1in}
\section{Comparisons to Synthetic Distribution Shifts (Demographic Parity)} \label{sec:syntheticcomparison}

To further interpret our results, in this section, we consider specific and popular agent models to characterize distribution shift and instantiate our bounds \rr{for particular forms of \(\mathbf{D}\), \(\mathbf{B}\), and \(\disp\)}. 

\subsection{Covariate Shift via Strategic Response} 
\label{sec:strategic-response} Let us consider a specific example of covariate
shift (\cref{eq:def-covariate-shift}) caused by a deterministic,
% \yc{non-deterministic?}
group-independent model of \emph{strategic response} in which agents react to a binary classification policy \(\pi\) characterized by
group-specific feature thresholds:
% in w from a particular group $g$ with the same feature $X = x$ all share the same probability of being truly qualified (or unqualified),
% %\rr{conditioned on group, right?} ($P(Y|X=x)$)
% and this functional relationship between $Y$ and $X$ remains unchanged despite the agent's response to the classifier.
\begin{equation}
  \hat{Y} \sim \pi(x, g) = \begin{cases}
  1 &\text{ with probability } 1 \text{ if } x \geq \tau_{g} \\
  0 &\text{ with probability } 1 \text{ otherwise }
\end{cases}
\end{equation}
%where we will assume feature domain \(\mathcal{X} = [0, 1]\).

% \paragraph{Setup} \rr{we can ignore the classifier as a player, and treat $\tau$ as given, right?} We formulate a two-player sequential game to model the interaction between a decision maker and strategic individuals.
% Consider a simple case in which each individual is associated with a single continuous feature $x \in \mathcal{X}$, a group membership $g\in G = \{a, b\}$ and a binary true qualification $y(x)\in \{0,1\}$, where $y(x)$ is a function of the feature vector $x$.

% A decision maker makes a binary decision  ($0$ as being reject and $1$ as being accept) for an individual using a group-dependent threshold policy of the form:
% \begin{align}
%     \pi_g(x) = \Indicator [x\geq \tau_g], ~ g\in \{a, b\}
% \end{align}
For simplicity, we assume the feature domain \(\mathcal{X} = [0, 1]\).
In response to threshold \(\tau_g\), agents in each group \(g\) may modify their feature \(x\) to \(x'\) by incurring a cost $c_g(x, x')\geq 0$. Similar to
\cite{hardt2016strategic}, we define the \emph{utility} \(u_g\) for agents in group \(g\) to be
\begin{align} \label{eq:strategic-utility}
  u_g(x, x') &\define \beta_g(x') - \beta_{g}(x) - c_g(x, x'); \quad \beta_{g}(x) \define \Pr(\hat{Y} {=} 1 \mid X {=} x, G {=} g),   \forall g.
\end{align}
Contrary to the standard strategic classification setting, we do not assume that
feature updates represent false reports, but that such updates may correspond to actual changes underlying the true qualification \(Y\)
of each agent. This assumption has been made in a recent line of research in
incentivizing improvement from human agents subject to such classification
\cite{chen2021linear}.

Next, we assume all agents are rational utility maximizers (\cref{eq:strategic-utility}).
% Because
% $\beta_g(x') - \beta_g(x) \leq 1$, agents will only attempt change their feature
% when $c_g(x, x') \leq 1$; and agent will not change their feature if
% $\beta_g(x) = 1$ (they are already been accepted with their original feature $x$).
For a given threshold $\tau_g$ and manipulation budget $m_{g}$, the best response
of an agent with original feature $x$ is
\begin{equation}
  x' = \argmax_{z}\ u_g(x, z), \quad \text{ such that }\ c_g(x, z) \leq m_{g}
\end{equation}
% Consider a simple case where the feature space is bounded $\mathcal{X}$ $:= [0,1]$, and the feature distribution follows a uniform distribution:
% \begin{align*}
%     \Pr_\S(x) =
%     \begin{cases}
%     1, \ \ & x\in [0, 1]\\
%     0,  & \text{otherwise}
%     \end{cases}
% \end{align*}
% With some additional assumptions about the agents' best response behaviors (\Cref{assumption:cost-function} ~-~ \Cref{assumption:new-feature-uniform-distribution} in \Cref{sec:proof-strategic-response}) 
To make the problem tractable, we make additional assumptions about the agents' best responses. 
\begin{assumption}
    An agent's original feature $x$ is sampled as $X\sim \mathcal{U}_{[0,1]}$\footnote{where \(\mathcal{U}\) represents the uniform distribution.}.
\end{assumption}
\begin{assumption}
\label{assumption:cost-function}
The cost function $c_g(x, x')$ is  monotone in $|x - x'|$ as
\(
  c_g(x, x') =  |x' - x|
\).
\end{assumption}
Under \Cref{assumption:cost-function}, only those agents with features
$x \in [\tau_g - m_{g}, \tau_g)$ will \emph{attempt} to change their feature. We
also assume that feature updates are non-deterministic, such that agents with
features closer to the decision boundary \(\tau_{g}\) have a greater
\emph{chance} of updating their feature and each updated feature \(x'\) is
sampled from a uniform distribution depending on \(\tau_{g}\), \(m_{g}\), and \(x\):

\begin{assumption} 
\label{assumption:nondeterministic-feature-update}
For agents who \emph{attempt} to update their features, the probability of
a successful feature update is
\(
    \Pr(X \neq X') = 1 - \frac{|x - \tau_g|}{m_{g}}
\).
\end{assumption}
% Intuitively this means that the closer the agent's original feature $x$ is to the decision boundary $\tau_g$, the more likely they can successfully change their feature to cross the decision boundary.



\begin{assumption}
\label{assumption:new-feature-uniform-distribution}
  An agent's updated feature \(x'\), given original feature \(x\), manipulation
  budget \(m_{g}\), and classification boundary \(\tau_{g}\), is sampled as
  \(
    X' \sim \mathcal{U}_{[\tau_g, \tau_g + m_{g} - x]}
  \).
%   where \(\mathcal{U}\) represents the uniform distribution.
    % Agent who starts at a particular feature $x\in [\tau_g - M_g, \tau_g]$ and successfully pass the decision boundary will have their new feature uniformly distributed between $[\tau_g, \tau_g + M_g - x]$.
\end{assumption}


With the above setting, we can specify the reweighting coefficient $\omega_g(x)$ for our setting (\cref{eq:strategic-omega} in \cref{sec:proof-strategic-response} and get the following bound for the strategic response setting\footnote{See \Cref{fig:sc-distribution-shift} in Appendix \ref{secA:additional-figures} for a demonstration of  \Cref{thm:dp-covariate}.}: 
% We obtain the following fairness violation bound for the strategic response case:
\begin{proposition}
  \label{proposition:bound-strategic-response}
  For our assumed setting of strategic response involving \DP for two groups \(\{g, h\}\),
\cref{thm:dp-covariate} implies
\vspace{-0.1in}
\begin{equation}
    \dispdp(\pi, \R) 
    %\leq & \disp(\pi, \S) + \Pr_{\S}(\pi_g(x) = +1) \var_{\S}(\omega_g(x)) + \Pr_{\S}(\pi_h(x) = +1) \var_{\S}(\omega_h(x))\\
    \leq \dispdp(\pi, \S) + \tau_g(1-\tau_g)\frac{2}{3}m_{g}  +
    \tau_h(1 - \tau_h)\frac{2}{3}m_{h}
\end{equation}
\end{proposition}
%\vspace{-0.1in}
The above result shows that two factors lead to a smaller difference between the source and target fairness violations: a less stochastic classifier (when the threshold $\tau_g$ is far away from $0.5$) and a smaller manipulation budget $m_g$ (diminishing agents' ability to adapt their feature). In this case, $B_g =\frac{2}{3} \tau_g (1 - \tau_g)$.
These factors lead to less potential manipulation and result in a tighter upper bound for the fairness violation on \(\R\).
% larger tau: tigher bound
% smaller manipulation budget, tigher bound
\vspace{-0.1in}
\begin{figure}
    \subfigure[A stereoscopic (cross-eye view) comparison between the bound of \cref{sec:covariateDP} (gradated) and simulated results for the model of \cref{sec:strategic-response} (blue) in response to a \DP-fair classifier with different initial group-independent acceptance rates. \label{fig:DP-covariate-experimental-small}]{\includegraphics[width=0.48\linewidth]{images/DP_bound.pdf}}
  %\caption{A stereoscopic (cross-eye view) comparison between the bound of \cref{sec:covariateDP} (gradated) and simulated results for the model of \cref{sec:strategic-response} (blue) in response to a \DP-fair classifier. A larger version, \cref{fig:DP-covariate-experimental}, is provided in \cref{secA:additional-figures} in the supplementary material.}
\hfill
\subfigure[\small{A policy satisfying \DP is subject to distribution shift prescribed by replicator dynamics (\cref{sec:replicator}). Realized disparity increases (blue) are compared to the theoretical bound (\cref{thm:dp-label}, gradated), which is tight when group have dissimilar qualification rates.}\label{fig:dp-replicator}  ]{\includegraphics[width=0.48\linewidth]{images/transfer.pdf}}
% \begin{subfigure}[t]{0.48\linewidth}
%   \includegraphics[width=\linewidth]{images/transfer.pdf}
%   %\vspace{-0.2in}
%   %\caption{A policy satisfying \DP is subject to distribution
% % shift prescribed by replicator dynamics. The local change in
% % qualification rates subject to this policy follows the streamlines,
% % while the local change in \(\dispdp\) is represented with color and
% % compared to the theoretical bound (\cref{thm:dp-label}).}

% \end{subfigure}
\caption{Comparisons to synthetic distribution. Larger versions are provided in \cref{sec:empirical-evals}.}
\end{figure}


% \yc{Case 2.2: when $\tau_g + B_g > 1$: move to appendix}\\


\subsection{Label Shift via Replicator Dynamics} \label{sec:replicator}

We now evaluate our theoretical bound for demographic
parity subject to label shift (\cref{thm:dp-label}) on the replicator dynamics model of
\citet{raab2021unintended}. \rev{Briefly, replicator dynamics assumes that the proportion of agents in a population choosing one strategy over another grows in proportion to the ratio of average utilities realized by the two strategies.
} The cited model additionally assumes \(\mathcal{X} = \RR\),
\(\mathcal{Y} = \{\FP\}\), and a monotonicity condition for \(\S\) given by
\(
    \dv{}{x} \frac{\Pr_{\S}(X {=} x \mid Y {=} 1)}{\Pr_{\S}(X {=} x \mid Y {=} 0)} > 0
\).

Label shift under the discrete-time (\(t\)) replicator dynamics may be expressed
in terms of group \emph{qualification rates}
\(Q_{g} \define \Pr_{t}(Y {=} 1 \mid G {=} g)\) and agent utilities
(\ie, group- and feature-independent values \(U_{y,\hat{y}}\)) such
that, in each group, the popularity and average utility associated with a label determines
its frequency at the next time step \(t{+}1\).

Denote the \emph{fractions} of group-conditioned, feature-independent outcomes with the expression
\(\rho^{y,\hat{y}}_{g} \define \Pr_{t}(\hat{Y} {=} \hat{y}, Y {=} y \mid G {=} g)\)
and abbreviate the fraction-weighted utility as
\(u^{y,\hat{y}}_{g}(t) \define U_{y,\hat{y}} \cdot \rho^{y,\hat{y}}_{g}\). We may then
represent the replicator dynamics as
\begin{align} \label{eq:replicator-dynamics}
  Q_{g}[t + 1] &= \frac{u^{\TP}_{g}(t) + u^{\FN}_{g}(t) } {u^{\TP}_{g}(t) + u^{\FN}_{g}(t) +  u^{\TN}_{g}(t) + u^{\FP}_{g}(t) }
\end{align}
To apply \cref{thm:dp-label}, we also observe that
$
  | \beta^{+}_{g} - \beta^{-}_{g} | = \frac{| \rho^{\TP}_{g} - \rho^{\FP}_{g} |}{\rho^{\TP}_{g} + \rho^{\FP}_{g}},
$
where \(\beta^{+}_{g}\) and \(\beta^{-}_{g}\) represent the true positive rate
and false positive rate for group \(g\), respectively, and we use the change in
qualification rate as our measurement of label shift, \ie,
\(B_{g} = |Q_{g}[t + 1] - Q_{g}[t]|\).
When demographic parity is perfectly
satisfied, we note that the acceptance rate
(\(\rho^{\TP}_{g} + \rho^{\FP}_{g}\)) is group-independent.

\begin{theorem}
  \label{thm:label-replicator}
  For \DP subject to label replicator dynamics,
  \begin{equation} \label{eq:dp-replicator-bound}
  \begin{aligned}
\dispdp(\pi, \R) \leq \dispdp(\pi, \S) + \sum_g \Big|Q_{g}[t + 1] - Q_{g}[t]\Big| \frac{| \rho^{\TP}_{g} - \rho^{\FP}_{g} |}{\rho^{\TP}_{g} + \rho^{\FP}_{g}}
  \end{aligned}
\end{equation}
\end{theorem}
% \yl{the previous bounds dont carry the absolute value but this one does; needs to unify. }
% \cref{eq:dplabelbound} evaluates to
% \begin{equation}
%     \Big|  \dispdp(\pi, \R) - \dispdp(\pi, \S) \Big|
%     \leq \sum_g
% \Big(\Big| \frac{U_{\TP}\TP_{g} + U_{\FN}\FN_{g} } {U_{\TP} \TP_{g} + U_{\FN} \FN_{g} +  U_{\TN} \TN_{} + U_{\FP} \FP_{g} } - s_{g} \Big|\Big)
% | \frac{\FP}{\FP + \TN} - \frac{\TP}{\TP + \FN} |
% \end{equation}
\vspace{-0.1in}
In \cref{fig:dp-replicator}, we graphically represent all possible states of an initially
fair system (thus determining \(\beta\) and \(\rho\) as a result of
the monotonicity condition) by the tuple of qualification rates for each group. With
the dynamics prescribed by \cref{eq:replicator-dynamics}, we depict the \emph{rate of change} of disparity given a fixed, locally \DP-fair policy, and compare this to the theoretical bound when \(B_{g} = |Q_{g}[t + 1] - Q_{g}[t]|\).

Interpreting our results, we note that the bound lacks information about the relative directions of the change in acceptance rates for each group, and thus over-approximates possible fairness violations when group acceptance rates shift the same direction. When group acceptance rates move in opposing directions, however, the bound gives excellent agreement with the modelled replicator dynamics.
% \iffalse
% \begin{figure}[!thb]
%     \centering
%     \subfigure[California $\longrightarrow$ Alaska]{\includegraphics[width=0.48\linewidth]{Simulation/CovariateShift/covariate_shift_CA_AK_2018.pdf}}
%     % \begin{subfigure}[b]{0.3\linewidth}
%     %     \includegraphics[width=\linewidth]{Simulation/CovariateShift/covariate_shift_CA_AK_2018.pdf}
%     %     \caption{California $\longrightarrow$ Alaska}
%     % \end{subfigure}
%     \hfill
%     % \begin{subfigure}[b]{0.3\linewidth}
%     %     \includegraphics[width=\linewidth]{Simulation/CovariateShift/covariate_shift_CA_IL_2018.pdf}
%     %     \caption{California $\longrightarrow$ Illinois}
%     % \end{subfigure}
%     \subfigure[California $\longrightarrow$ Illinois]{\includegraphics[width=0.48\linewidth]{Simulation/CovariateShift/covariate_shift_CA_IL_2018.pdf}}
%     \hfill
%     % \begin{subfigure}[b]{0.3\linewidth}
%     %     \includegraphics[width=\linewidth]{Simulation/CovariateShift/covariate_shift_CA_NV_2018.pdf}
%     %     \caption{California $\longrightarrow$ Nevada}
%     % \end{subfigure}
%     % \subfigure[California $\longrightarrow$ Nevada]{\includegraphics[width=0.3\linewidth]{Simulation/CovariateShift/covariate_shift_CA_NV_2018.pdf}}
%     \caption{Modelled change in \DP violation subject to geographic distribution shift (California to other US states) \vs direct application of \cref{thm:dp-covariate} without establishing covariate shift. The $x$-axis and $y$-axis represent the thresholds $\tau_g$ and $\tau_h$, respectively used to train the policy.}
%     \label{fig:covariate_shift_CA}
% \end{figure}

% \begin{figure}[!thb]
%     \centering
%     % \begin{subfigure}[b]{0.3\linewidth}
%     %     \includegraphics[width=\linewidth]{Simulation/LabelShift/label_shift_CA_2014_2018.pdf}
%     %     \caption{California}
%     % \end{subfigure}
%     %\subfigure[California]{\includegraphics[width=0.48\linewidth]{Simulation/LabelShift/label_shift_CA_2014_2018.pdf}}
%     \hfill
%     % \begin{subfigure}[b]{0.3\linewidth}
%     %     \includegraphics[width=\linewidth]{Simulation/LabelShift/label_shift_MA_2014_2018.pdf}
%     %     \caption{Massachusetts}
%     % \end{subfigure}
%     \subfigure[Massachusetts]{\includegraphics[width=0.48\linewidth]{Simulation/LabelShift/label_shift_MA_2014_2018.pdf}}
%     \hfill
%     %\begin{subfigure}[b]{0.3\linewidth}
%     %     \includegraphics[width=\linewidth]{Simulation/LabelShift/label_shift_TX_2014_2018.pdf}
%     %     \caption{Texas}
%     % \end{subfigure}
%     \subfigure[Texas]{\includegraphics[width=0.48\linewidth]{Simulation/LabelShift/label_shift_TX_2014_2018.pdf}}
%     \caption{Modelled change in \DP violation subject to temporal distribution shift (2014 to 2018) \vs direct application of \cref{thm:dp-label} without establishing label shift. The $x$-axis and $y$-axis represent the thresholds $\tau_g$ and $\tau_h$, respectively used to train the policy.}
%     \label{fig:label_shift_temporal_CA}
% \end{figure}
% \fi
\vspace{-0.1in}
\section{Comparisons to Real-World Distribution Shifts} \label{sec:realcomparison}
\vspace{-0.1 in}
We now compare our special-case theoretical bounds \rev{(\ie, label/covariate shift)} to real-world distribution
shifts and hypothetical classifiers. We use American Community Survey (ACS) data
provided by the US Census Bureau \cite{IPUMS}. We adopt the sampling and
pre-processing approaches following the \texttt{Folktables} package provided by
\citet{ding2021retiring}\footnote{This package is available at
\url{https://github.com/zykls/folktables}.} to obtain 1,599,229 data points. The
data is partitioned by (1) all fifty US states and (2) years from 2014 to
2018. We use 10 features covering the demographic information used in the UCI
Adult dataset \cite{Blake1998UCIRO}, including age, occupation, education, \etc,
as \(X\) for our model, select sex as binary protected group, i.e.,
\(G \in \{g=\texttt{female}, h=\texttt{male}\}\). We set the label \(Y\) to whether an individual's annual income is greater than \$50K. 

\rev{To apply our label-shift or covariate-shift bounds, we first need to verify whether the two datasets satisfy either of these assumptions. }
We adopted a conditional independence test \cite{NEURIPS2020_e2d52448}, \rev{which takes data from source and target domains as input and returns a divergence score for each covariate and label variable, reflecting to what extent the variable is shifted between distributions.} We find that the likelihood that the covariates shift across US states is approximately two orders of magnitude higher than for labels.
%\yl{can we add some numbers for this test?}\jw{I rephrased this paragraph and added the numbers}. 
 More specifically, there are 4 covariates, including class of worker (probabilistic divergence score of 2.67e-2), hours worker per week (3.56e-2), sex (3.56e-2) and race (2.55e-1), that are more likely to be shifted than the label variable (1.29e-4). For temporal shifts within states, \rev{we find that the label variable is more likely to be shifted (0.1) than all the other covariates (which are below 0.01), approximately two orders of magnitude in favor of label shift over covariate shift. We therefore compare the disparities of hypothetical policies on these distributions to bounds generated from the corresponding, approximately satisfied assumptions.}

On this data, we train a set of group-dependent, linear threshold
classifiers $\Pr_{\pi(x, g)}(\hat{Y} {=} 1) = \Indicator[\sigma(w \cdot x) > \tau_g]$,
for a range of thresholds \(\tau_{g}\) and \(\tau_{h}\) for each source
distribution. Here, $\sigma(\cdot)$ is the logistic function and $w$ denotes a
weight vector. We then consider two types of real-world distribution shift: (1)
\emph{geographic}, in which a model trained for one state is
evaluated on other US state in the same year, and (2) \emph{temporal}, in which a model trained for 2014 is evaluated on the same
state in 2018.
%take data examples in the year of 2014 as source distribution and those in the year of 2018 as target distribution.

% We assume that groups $g$ and $h$ have different thresholds $\tau_g$
% and $\tau_h$ for imposing fairness constraints.
% For this study, we take
% demographic parity as the fairness constraint.

% We apply threshold classifier models to data that varies by US state and year
% (2014 or 2018). Varying the thresholds $\tau_g$ and $\tau_h$, we obtain a series
% of linear classifiers with different fairness violations on the target
% distribution.
\vspace{-0.2in}
\begin{figure}[H]
    \centering
    \subfigure[CA $\longrightarrow$ IL]{\includegraphics[width=0.24\linewidth]{Simulation/CovariateShift/covariate_shift_CA_IL_2018.pdf}}
    \subfigure[CA $\longrightarrow$ NV]{\label{fig:simulation-state-ca-nv}\includegraphics[width=0.24\linewidth]{Simulation/CovariateShift/covariate_shift_CA_NV_2018.pdf}}
    \subfigure[CA: 2014 $\rightarrow$ 2018]{\label{fig:simulation-time-ca}\includegraphics[width=0.24\linewidth]{Simulation/LabelShift/label_shift_CA_2014_2018.pdf}}
    \subfigure[TX: 2014 $\rightarrow$ 2018]{\label{fig:simulation-time-tx}\includegraphics[width=0.24\linewidth]{Simulation/LabelShift/label_shift_TX_2014_2018.pdf}}
    \caption{Simulated change in \DP violation \rev{(blue mesh)} subject to geographic and temporal distribution shifts \vs direct application of bounds for approximately satisfied assumptions (respectively, \cref{thm:dp-covariate} and \cref{thm:dp-label}) \rev{(gradated mesh)}. The $x$-axis and $y$-axis of both figures represent the policy thresholds $\tau_g$ and $\tau_h$.}
    \label{fig:combined_simulation}
    \vspace{-0.1in}
\end{figure}
% \yl{need to double check the negative change of violations in the figures}
We graphically compare the theoretical bounds of
\cref{thm:dp-covariate} and \cref{thm:dp-label} for the increased violation of
\DP subject to covariate and label shift, respectively, to the simulated
violations for our model and data in \cref{fig:combined_simulation}. \rev{We provide additional examples and an evaluation of bounds for \EO subject to covariate shift (noting that label shift preserves \EO in theory) in \cref{app:real-world-data}. Despite the fact that geographic or
temporal distribution shifts only approximately satisfy the assumptions of
covariate or label shift, these comparisons demonstrate that our theoretical bounds are not vacuous, approximately bounding the change of fairness violation across real-world domain shifts. For geographic shifts, the covariate shift \EO bounds (\cref{app:real-world-data}) correctly overestimate disparity and tighten near accurate policies, while our \DP bounds are useful only for a subset of policy thresholds (Figure \ref{fig:simulation-state-ca-nv}). {add specific pointer. e.g, 4.a, that one is 4.b} For temporal shift, the label shift bound for \DP correctly overestimates the real change of DP violations but still remains at the same order of magnitude (Figure \ref{fig:simulation-time-ca} and \ref{fig:simulation-time-tx}).}

% are interested in two quantities: (1) the modelled change in \DP violation as
% the underlying distribution shifts, either in state, or in year, and (2) the
% theoretical upper bounds for covariate or label shift. We plot the change in
% \DP violation under geographic distribution shift with California as the source
% state in \cref{fig:covariate_shift_CA}. The blue surface represents the
% estimated upper bound subject to covariate shift, and the gradated surface
% represents the realized change of fairness violation evaluated between different
% states. We use \(\tau_{g}\) and \(\tau_{h}\) as our axes, thus evaluating our
% bounds even when the classifier is unfair on the source distribution. We calculate the upper bounds by applying \cref{thm:dp-covariate}.
% We observe that the theoretical upper bound for covariate shift is approximately applicable.

% Likewise, we plot the simulated change to \DP violation under
% temporal distribution shift in \cref{fig:label_shift_temporal_CA} for different
% states, compared to the label shift bounds. We apply \cref{thm:dp-label} to measure the upper bounds. We find that the label shift bounds generally apply to modelled temporal shifts.

% \rr{Must comment on how we measure \(D_g\) for shifts that do not adhere to assumptions.}
% We do recognize our label shift bound fails for some choices of
% parameters $\tau_g$ and $\tau_h$ in California, but it can perfectly fit the
% Massachusetts and Texas partitions for temporal distribution shift. To sum up,
% the upper bounds posed in our work are capable of satisfying the real-world
% distribution shift.


==> Fairness Transfer Bounds-ArXiv3/Section/TargetShift.tex <==
\section{Label Shift} \label{sec:labelDP}
\vspace{-0.1in}
Under label shift (\(\Pr_\S(X|Y) = \Pr_\R(X|Y)\)), violations of \EO and \EOp are invariant, because
the independence of \(\hat{Y}\) and \(Y\) given \(X\)
implies
$\Pr_{\pi,\R}(\hat{Y}|Y) = \Pr_{\pi,\S}(\hat{Y}|Y)$. We therefore focus on the violation of
demographic parity (\DP) (\cref{eq:def-demographic-parity}) subject to the label shift condition, treating a binary
classification task over two groups for simplicity.

In this setting, we choose to measure group-specific distribution shifts \rr{from}
\(\S\) \rr{to} \(\R\) by the change in proportion of \rr{ground-truth} positive labels, which we
refer to as the group \emph{qualification rate}
\(Q_{g}(\R) \define  \Pr_\R(Y = 1 \mid G = g)\):
\begin{align} \label{eq:defDlabelDP}
  D_{g}(\R \parallel \S) \define \Big| Q_{g}(\mathcal{S}) - Q_{g}(\mathcal{\R}) \Big| \leq B_{g}
\end{align}
% The realized value of \(\dispdp\), subject
% to distribution shift \(\S \mapsto \R\), is bounded by the
% group-subadditive condition (\cref{sec:groupsubadditivity})
% \begin{align}
%   \dispdp(\pi, \R) \leq v(\pi, \S, \mathbf{B}) \leq \tilde{v}(\pi, \S, \mathbf{B})
% \end{align}
% where
% \begin{align}
%   \tilde{v}(\pi, \S, \mathbf{B}) \define
%   \dispdp(\pi, \S) +
%   \sup_{ \mathbf{D}(\R \parallel \S) \preceq \mathbf{B}} \sum_{g} \Big|\Pr_\R(\hat{Y} = +1 \mid G = g) - \Pr_\mathcal{\S}(\hat{Y}= +1 \mid G = g) \Big|
% \end{align}
\begin{theorem} \label{thm:yangsthm}
A Lipshitz condition bounds \(\nabla_\mathbf{b} v(\disp_\DP, \mathbf{D}, \pi, \S, \mathbf{b})\) when
\begin{equation}
    D_{g}(\R \parallel \S) \define \Big| Q_{g}(\mathcal{S}) - Q_{g}(\mathcal{\R}) \Big| \leq B_{g}
\end{equation}
Specifically,
\begin{equation}
  \pdv{}{b_{g}} v(\disp_\DP, \mathbf{D}, \pi, \S, \mathbf{b}) \leq
  (|\mathcal{G}| - 1)
  \Big| \beta^{+}_{g} - \beta^{-}_{g} \Big|
\end{equation}
for true positive rates \(\beta^{+}_{g}\) and false positive rates \(\beta^{-}_{g}\):
\begin{equation}
    \beta^{+}_{g}
\define \Pr_{\pi}( \hat{Y} {=} 1 \mid Y {=} 1, G {=} g ); \quad \beta^{-}_{g} \define \Pr_{\pi}( \hat{Y} {=} 1 \mid Y {=} 0, G {=} g )
\end{equation} 
\end{theorem}
% In \cref{thm:yangsthm}, the absolute difference between the true positive rate \(\beta^{+}_g\)
% and false positive rate \(\beta^{-}_g\) of classifier policy \(\pi\) on group
% \(g\) bounds the rate of change in \(\disp_\DP\) for two groups subject to
% distribution shift measured by \(D_{g}\) (\cref{eq:defDlabelDP}).
Because \(\beta^{+}_g\) and \(\beta^{-}_g\) are invariant under label shift
given a constant policy \(\pi\), we elide their explicit dependence on the underlying distribution.
% \yc{notations of $\beta_g^+$ and $\beta_g^-$? Shall we use standard notation
% like $\TPR$ and $\FPR$ instead?}\rr{I thought about this. I prefer the \(\beta\)
% notation for compactness and consistency with, \eg, Section 2, but if you are
% strongly opposed, I am open to reconsideration.}

% We next observe that each component of \(\mathbf{D}\) is symmetric in its
% arguments, and therefore a metric. From \rr{Remove Lower Bound language}, we obtain
% both an upper and a lower bound on \(\disp(\pi, \R)\):
\begin{theorem}\label{thm:dp-label}
For \DP under the bounded label-shift assumption $\forall g,  | Q_{g}(\S) - Q_{g}(\R) | \leq B_{g}$,
% \yc{LHS should just be \(\disp(\pi, \R) -\disp(\pi, \S) \)?}
\begin{equation}
\begin{aligned} \label{eq:dplabelbound}
 \dispdp(\pi, \R)  &\leq  \dispdp(\pi, \S) + (|\mathcal{G}| - 1)
\sum_g B_{g} \ \Big|\beta^{+}_g - \beta^{-}_g \Big|
\end{aligned}
\end{equation}
\end{theorem}
\vspace{-0.15in}
Intuitively, the change in \(\disp_\DP\) subject to label shift \rr{depends on} \(|\beta^{+}_{g} - \beta^{-}_{g}|\), the marginal change in acceptance rates as agents change their qualifications \(Y\).
\rr{We measure the distribution shift as agents change their qualifications} by \(|Q_g(\S) - Q_g(\R)|\). When
$\beta^{+}_{g}$ is close to $\beta^{-}_{g}$, the policy looks like a random
classifier, and a label shift has limited effect on statistical group disparity.
When $|\beta^{+}_{g} - \beta^{-}_{g}|$ is large, indicating high classifier
accuracy, the effect \rr{on supremal disparity} is larger. Our bound thus exposes a direct trade-off between accuracy and fairness
transferability guarantees.


==> Fairness Transfer Bounds-ArXiv3/macros.tex <==
\usepackage[english]{babel} % inform standard packages of language used
% \usepackage[T1]{fontenc}    % use 8-bit T1 fonts for output.  NOT COMPATIBLE WITH ACMART
\usepackage[utf8]{inputenc} % allow utf-8 input

% Fonts and Colors
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{dsfont}         % for e.g., indicator function
\usepackage{bm}             % bold symbols
\usepackage{xcolor}         % colors
\usepackage{xspace}         % smart whitespace for text macros

% Maths
\usepackage[]{amsthm}       % proof, theorem, lemma, etc. environments
% \usepackage[]{amssymb}      % A bunch of math symbols
\usepackage[]{mathtools}    % loads amsmath

% Physics
% http://mirrors.ibiblio.org/CTAN/macros/latex/contrib/physics/physics.pdf
\usepackage{physics}

% syntax highlighting
% \usepackage{minted}
% \usemintedstyle{monokai}
% \usepackage{sourcecodepro}

% Diagrams, Tables, Graphics
\usepackage{booktabs}       % professional-quality tables
\usepackage{graphicx}       % for figures
\usepackage[]{tikz}         % for drawing figures
\usepackage[]{pgfplots}     % for drawing figures
\usepackage{float}          % placing figures
\usepackage{wrapfig}        % placing figures
%\usepackage[font={normalsize}]{caption}
\usepackage{caption}
% \usepackage{subcaption}     % subfigures not compatible with subfigure

% Subcaptions include figure number
% \makeatletter
% \newcommand\nocaption{%
%     \renewcommand\p@subfigure{}
%     \renewcommand\thesubfigure{\thefigure\alph{subfigure}}
% }
% \makeatother

% Links & Counter
\usepackage{url}                               % simple URL typesetting
\usepackage{hyperref}                          % hyperlinks
% \usepackage[capitalize, nameinlink]{cleveref}  % references to equations, sections, etc. imported
\usepackage{crossreftools}
\pdfstringdefDisableCommands{%
  \let\Cref\crtCref
  \let\cref\crtcref
}
\crefformat{footnote}{#2\footnotemark[#1]#3} % footnote style for cref
\usepackage{refcount}                        % Set counter by reference

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Lemma-Theorem-Proof structure envorinments
\iffalse
\newcommand{\renewtheorem}[1]{%
  \expandafter\let\csname #1\endcsname\relax
  \expandafter\let\csname c@#1\endcsname\relax
  \expandafter\let\csname end#1\endcsname\relax
  \newtheorem{#1}%
}

\theoremstyle{plain}

\renewtheorem{thm}{Theorem}
\renewtheorem{cor}{Corollary}[thm]
\renewtheorem{lem}{Lemma}[thm]
\renewtheorem{obs}{Observation}[thm]
\renewtheorem{fact}{Fact}[thm]
\renewtheorem{prop}[thm]{Proposition}
\renewtheorem{asm}{Assumption}

% the following environments keep the roman font:
\theoremstyle{definition}

\renewtheorem{rem}[thm]{Remark}
\renewtheorem{rems}[thm]{Remarks}
\renewtheorem{exa}[thm]{Example}
\renewtheorem{exas}[thm]{Examples}
\renewtheorem{defi}[thm]{Definition}
\renewtheorem{conv}[thm]{Convention}
\renewtheorem{conj}[thm]{Conjecture}
\renewtheorem{prob}[thm]{Problem}
\renewtheorem{oprob}[thm]{Open Problem}
\renewtheorem{algo}[thm]{Algorithm}
\renewtheorem{qu}[thm]{Question}
\renewtheorem{pty}[thm]{Property}
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%n

% Proof environment with line to the left
\usepackage[many]{tcolorbox}
\tcolorboxenvironment{proof}{
  blanker,
  before skip=12pt,
  after skip=12pt,
  borderline west={0.4pt}{0.4pt}{black},
  breakable,
  left=8pt,
}
\renewcommand\qedsymbol{}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%n
% Math
\newcommand{\define}{\coloneqq}
\newcommand{\nimplies}{\centernot\implies}

% integration / differentiation
% See http://mirrors.ibiblio.org/CTAN/macros/latex/contrib/physics/physics.pdf

% Probability
% \Pr already included
\newcommand{\avg}{\overline} % avergage
\newcommand{\pr}{p} % Probability density (can also be f)
\DeclareMathOperator*{\E}{\mathbb{E}} % Expectation value
\DeclareMathOperator*{\I}{\text{I}}   % Mutual Information
\DeclareMathOperator*{\HH}{\text{H}}  % Information Entropy
%\renewcommand{\cov}{\operatorname*{Cov}}

% More functions
\newcommand{\1}[1]{\mathbf{1}_{#1}} % indicator function
\newcommand{\Indicator}{\mathds{1}}
\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\argmin}{argmin}
%% \DeclareMathOperator*{\arclen}{arclen}
\newcommand{\sthat}{\text{such that }}
\newcommand{\subto}{\text{subject to }}
\DeclareMathOperator{\sign}{sgn}
\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}

% Standard Numerical Sets (Can be \mathbb, alternatively)
\newcommand{\PP}{\mathbf{P}} % primes
\newcommand{\NN}{\mathbf{N}} % naturals
\newcommand{\ZZ}{\mathbf{Z}} % integers
\newcommand{\QQ}{\mathbf{Q}} % rationals
\newcommand{\RR}{\mathbf{R}} % reals
\newcommand{\CC}{\mathbf{C}} % complex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Prosaic

% Latin Abbreviations
\newcommand{\NB}{\emph{Note}\xspace}  % Note well
\newcommand{\vs}{\emph{vs.}\xspace}   % Versus
\newcommand{\eg}{\emph{e.g.}\xspace}  % For example
\newcommand{\ie}{\emph{i.e.}\xspace}  % That is
\newcommand{\etc}{\emph{etc.}\xspace} % And so on
\newcommand{\cf}{\emph{cf.}\xspace}   % Compare with
\newcommand{\viz}{\emph{viz.}\xspace} % Namely

%% % Quoting
%% \let\oldquote\quote
%% \let\endoldquote\endquote
%% \renewenvironment{quote}[2][]
%%   {\if\relax\detokenize{#1}\relax
%%      \def\quoteauthor{#2}%
%%    \else
%%      \def\quoteauthor{#2~---~#1}%
%%    \fi
%%    \oldquote}
%%   {\par\nobreak\smallskip\hfill---\quoteauthor%
%%    \endoldquote\addvspace{\bigskipamount}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Editing

\usepackage{ulem}       % editing (sout)
\normalem               % prevent ulem from rendering \emph{} as underlined

% quote
\newcommand{\qt}[1]{``#1''}

